FLAC: A Robust Failure-Aware Atomic Commit Protocol for Distributed Transactions

In distributed transaction processing, atomic commit protocol (ACP) is used to ensure database consistency. With the use of commodity compute nodes and networks, failures such as system crashes and network partitioning are common. It is therefore important for ACP to dynamically adapt to the operating condition for efficiency while ensuring the consistency of the database. Existing ACPs often assume stable operating conditions, hence, they are either non-generalizable to different environments or slow in practice. In this paper, we propose a novel and practical ACP, called Failure-Aware Atomic Commit (FLAC). In essence, FLAC includes three protocols, which are specifically designed for three different environments: (i) no failure occurs, (ii) participant nodes might crash but there is no delayed connection, or (iii) both crashed nodes and delayed connection can occur. It models these environments as the failure-free, crash-failure, and network-failure robustness levels. During its operation, FLAC can monitor if any failure occurs and dynamically switch to operate the most suitable protocol, using a robustness level state machine, whose parameters are fine-tuned by reinforcement learning. Consequently, it improves both the response time and throughput, and effectively handles nodes distributed across the Internet where crash and network failures might occur. We implement FLAC in a distributed transactional key-value storage system based on Google Percolator and evaluate its performance with both a micro benchmark and a macro benchmark of real workload. The results show that FLAC achieves up to 2.22x throughput improvement and 2.82x latency speedup, compared to existing ACPs for high-contention workloads.

==> chapters/formal-proof-of-correctness.tex <==
\phxsays{This will be replaced by a short proof of correct when submit to VLDB.}
\subsection{Proof of Correctness}
\label{sec:formalProof}

\subsubsection{FSA Model of ACP}

We follow existing works~\cite{Skeen, gupta2018easycommit, gray2006consensus} to model the transaction execution at each node as an \textbf{finite state automata} (FSA) and regards network messages as the inputs/outputs.
%
The state of FSA on node $i$ is called the \textbf{local state}.
%
For a state transition, the node reads nonempty strings of messages sent to it, writes strings of messages as output, and makes an instantaneous change to the local state.
%
The local state transitions are atomic without crash failures and performed asynchronously.

Figure~\ref{fig:prac-ff} and Figure~\ref{fig:prac-cf} separately present the FSA for {\flacFF} and {\flacCF} (Algorithms ~\ref{alg:CO1} ~\ref{alg:LP1} ~\ref{alg:CO2} and ~\ref{alg:LP2}).
%
Node 1 is fixed as the coordinator, while nodes 2 -- n represent involved participants.
%
We mark the event "a $MessageName$ message is sent from $u$ to $v$" as $MessageName_{u, v}$.
%
FSAs contain five basic states: \textbf{initial state} $q_i$, two \textbf{wait states} $w_i, r_i$, and two \textbf{final states} $c_i, a_i$ indicating the transaction is committed/aborted.
%
FSAs for {\flacCF} also contain two \textbf{buffer states}: a committable state $tc_i$ and an abortable state $ta_i$.
%
The two buffer states originals from the transmit-before-decide technique~\cite{gupta2018easycommit}, corresponding to the \textit{TRANSMIT-C} state and \textit{TRANSMIT-A} state of EasyCommit, respectively.
%
These FSAs are acyclic for eventual termination and are non-deterministic due to deadlocks, failures, triggers, or user aborts.
%
The messages sent between nodes can be reordered or delayed but can reach the destination before \textit{timeout} without crash failures.
%

\begin{figure}[ht]
  \centering
  \subfigure[Coordinator.]{%
    \includegraphics[width=0.8\linewidth]{figures/fsa-ff-co.png}
    \label{fig:fsa-ff-co}
  }
  \subfigure[Participant.]{%
    \includegraphics[width=0.8\linewidth]{figures/fsa-ff-pa.png}
    \label{fig:fsa-ff-pa}
  }
  %
  \caption{The FSA of {\flacFF}.}
  \label{fig:fsa-ff}
\end{figure}

Here we list some key definitions in Skeen's formalism~\cite{Skeen, gupta2018easycommit}.
%
The overall state of a distributed transaction $T$ can be defined as a combination of (i) a vector of all local states and (ii) the pending messages in the network, which is called the \textbf{global state}.
%
The global state is a \textbf{global final state} if all local states are final states.
%
The global state is a \textbf{global terminal state} if all local states are blocked and cannot transition to the following states.
%
Regarding a local state $x$, all local states that could concurrently exist with $x$ in reachable global states are called the \textbf{concurrency set} of $x$.
%
Finally, we call local states that can only exist when all participants have voted yes the \textbf{committable states}.
%
Otherwise, they are called \textbf{non-committable states}.
%


\begin{figure}[ht]
  \centering
  \subfigure[Coordinator.]{%
    \includegraphics[width=0.98\linewidth]{figures/fsa-cf-co.png}
    \label{fig:fsa-cf-co}
  }
  \subfigure[Participant.]{%
    \includegraphics[width=0.98\linewidth]{figures/fsa-cf-pa.png}
    \label{fig:fsa-cf-pa}
  }
  \caption{The FSA of {\flacCF} protocol.}
  \label{fig:fsa-cf}
\end{figure}

\subsubsection{Properties}

With the FSA model of ACPs, the atomic commit protocol correctness defined in Definition~\ref{def1} can be rewritten as Definition~\ref{def:fsa-acp}.

\begin{definition}
\label{def:fsa-acp}
    A commit protocol is a non-blocking atomic commit protocol if it ensures the following properties for global terminate states:
    \begin{itemize}
        \item The commit state is not in the concurrency set of the abort state.
        \item Only committable states can reach the commit state.
        \item A committable state must eventually transition to the commit state in a failure-free environment.
        \item All global terminal states are global final states.
    \end{itemize}
    They respectively correspond to the agreement, validity, and termination properties in Definition~\ref{def1}.
\end{definition}


% Other than them, Skeen provides two different properties for ACP FSA in distributed systems: \textit{non-deterministic} and \textit{eventual terminate}.
% %
% Non-deterministic describes the complexity of the atomic commit problem.
% %
% It claims that the behavior of each FSA cannot be predicted with deadlock, failures, or user aborts.
% %
% Moreover, the events for FSAs can be arbitrarily reordered, i.e., the message transition to each node can be received out-of-order.
%




\subsubsection{Sub-protocol Correctness}
\label{sec:subCorrectness}

The correctness of ACP can be described as a combination of agreement and validity properties.
%
We first present the correctness of {\flacFF} and {\flacCF}.
%
Based on Figure~\ref{fig:fsa-ff-pa} and ~\ref{fig:fsa-cf-pa}, we list concurrent sets of each state in Table~\ref{tab:concurrency-ff} and ~\ref{tab:concurrency-cf}.
%
For instance, $q_i$ does not concurrent with $c_j$ in Table~\ref{tab:concurrency-ff}, because the transition to $c_j$ requires $yes_{i,j}$, indicating $i$'s FSA has at least transited to $r_i$.
%
$q_i$ coexists with $w_j$ when the propose messages arrive node $j$ earlier than node $i$.
%
In this case, if node $j$ then votes {\no}, $q_i$ will coexist with $a_j$.
%
Note that $r_i$'s concurrency set is not listed in tables, because it can always transition and thus is not in any terminate state.
%
Among all states, $c_i$ of both protocols and $tc_i, w_i$ of {\flacCF} are committable states.
%

\begin{table}[ht]
  \centering
  \caption{{\flacFF} concurrency sets}
%  \vspace{-1em}
  \label{tab:concurrency-ff}
  
  \begin{tabular}{|c|c|c|c|c|}
  \hline
    & $q_j$ & $w_j$ & $a_j$ & $c_j$ \\
    \hline
    $q_i$ & \checkmark &  \checkmark &  \checkmark &  \\
  \hline
    $w_i$ & \checkmark &  \checkmark &  \checkmark & \checkmark  \\
  \hline
    $a_i$ & \checkmark &  \checkmark &  \checkmark & \\
  \hline
    $c_i$ & &  \checkmark & &  \checkmark \\
      \hline
  \end{tabular}
  
\end{table}

\begin{table}[ht]
  \centering
  \caption{{\flacCF} concurrency sets}
%  \vspace{-1em}
  \label{tab:concurrency-cf}
  
  \begin{tabular}{|c|c|c|c|c|c|c|}
  \hline
    & $q_j$ & $w_j$ & $ta_j$ & $tc_j$ & $a_j$ & $c_j$ \\
    \hline
    $q_i$ & \checkmark &  \checkmark & \checkmark & &  & \\
  \hline
    $w_i$ & \checkmark &  \checkmark &  \checkmark & \checkmark & &  \\
  \hline
    $ta_i$ & \checkmark &  \checkmark &  \checkmark &  & \checkmark &  \\
  \hline
    $tc_i$ &  &  \checkmark &  & \checkmark & & \checkmark \\
  \hline
    $a_i$ & & &  \checkmark & &  \checkmark & \\
  \hline
    $c_i$ & & & & \checkmark & &  \checkmark \\
      \hline
  \end{tabular}
  
\end{table}

%
In both tables, the commit state is not in the concurrency set of the abort state, ensuring the agreement property according to Definition~\ref{def:fsa-acp}.
%
The first node decides commit must be committable (collect all {\yes}), and thus ensures rule 2 (commit validity).
%
Rule 3 (abort validity) holds for $c_i$ in {\flacFF} and {\flacCF} since $c_i$ is already the final commit state.
%
Rule 3 for the rest committable states ($w_i, tc_i$ in {\flacCF}) can be proven by the following statements:
%
In a failure-free environment, the vote from each participant will reach the coordinator and results in a commit decision.
%
The commit decision then must reach all participants without network failure, inputting $commit_{1,i}$ to each FSA, transitioning them to $tc_i$, and committing transaction branches.
%
In all, committable states in both protocols ensure abort validity.

Another property of {\flac} mentioned in Section~\ref{LP2} is the liveness of {\flacCF}.
%
We reuse the fundamental non-blocking theorem~\cite{Skeen} to prove this part.
%
The theorem can be concluded as Theorem~\ref{the:nbac}.

\begin{theorem}[Fundamental non-blocking theorem.]
\label{the:nbac}
An ACP is non-blocking iff it ensures the following two conditions for participant FSAs:
%
(i) no local state is concurrent with both commit and abort states, and
%
(ii) no noncommittable state is concurrent with commit states.
\end{theorem}

It can be directly observed from Table~\ref{tab:concurrency-ff} and ~\ref{tab:concurrency-cf} that no state is concurrent with both $c_i$ and $a_i$, while $c_i$ is only concurrent with committable states $c_i$ and $tc_i$.
%
Thus, we can conclude that {\flacCF} ensures liveness regarding crash failures.

==> chapters/implementation.tex <==
\section{\pac\ Design}
\label{implementation}

\subsection{Components}

We implemented the code for \pac \ in Go, and the code for RL learner (which is included in \rlsm) in python. The implementation is available publicly on GitHub.~\cite{PAC}


\subsection{Message Upper Bound}
\label{factorr}

As demonstrated above, the message upper bound is defined as the sum of message passing time and local execution time. When implementing the system, a problem arises about how to select that value for the \pac \ protocol.
To reach theoretical optima, the waiting time for each cohort should be different and be tailored for each cohort. This can be done without lots of work on a stable network. However, if message delays between nodes keep changing, it would affect the performance. This reveals a natural trade-off between the requirement for network and the performance in \pac.
Specifically, we record the average of that message upper bound based on real executions and message delay between cohorts. Then we let the \pac \ protocol waits for $r$ ($r \ge 1$) times that result.
This $r$ represents how confident we are on the network stableness between cohorts. Section~\ref{exp} gives our evaluation in the trade-off on the selection of $r$ during experiments.

